Understanding Why ViT Trains Badly on Small Datasets: An Intuitive Perspective

Vision transformer (ViT) is an attention neural network architecture that is shown to be effective for computer vision tasks. However, compared to ResNet-18 with a similar number of parameters, ViT has a significantly lower evaluation accuracy when trained on small datasets. To facilitate studies in related fields, we provide a visual intuition to help understand why it is the case. We first compare the performance of the two models and confirm that ViT has less accuracy than ResNet-18 when trained on small datasets. We then interpret the results by showing attention map visualization for ViT and feature map visualization for ResNet-18. The difference is further analyzed through a representation similarity perspective. We conclude that the representation of ViT trained on small datasets is hugely different from ViT trained on large datasets, which may be the reason why the performance drops a lot on small datasets.

==> architecture.tex <==
\section{Model Architecture}

\begin{figure}[ht!]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Image/architecture/resnet18.pdf}
         \caption{ResNet-18, model size = 11.18M}
         \label{fig:resnet18}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Image/architecture/resnet14.pdf}
         \caption{ResNet-14, model size = 2.78M}
         \label{fig:resnet14}
     \end{subfigure}
     \vfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Image/architecture/wide_resnet14.pdf}
         \caption{Wide ResNet-14, model size = 4.66M}
         \label{fig:wide_resnet14}
     \end{subfigure}
        \caption{Network Architectures}
        \label{fig:three graphs}
\end{figure}


To design a ResNet architecture that fulfills the model size requirements, we start with the original ResNet-18 (Figure \ref{fig:resnet18}) architecture which has around 11.18M parameters. We first reduced the model size by removing the last residual layer and changing the average pooling kernel size from $4\times4$ to $8\times8$ accordingly. We kept all remaining parts the same and observe the model size for this ResNet-14 model is 2.78 M (Figure \ref{fig:resnet14}).

Empirical studies show that ResNet with wider channels can improve performance and efficiency without designing a very deep network \cite{wideresnet}. Motivated by this idea, we multiplied the channel size by around 1.3 times of the original channel size of the previous ResNet-14 model and made it our final model, Wide ResNet-14, which has 4.66M trainable parameters (Figure \ref{fig:wide_resnet14}). 







